CoMRAT: Commit Message Rationale Analysis Tool

In collaborative open-source development, the rationale for code changes is often captured in commit messages, making them a rich source of valuable information. However, research on rationale in commit messages remains limited. In this paper, we present CoMRAT, a tool for analyzing decision and rationale sentences rationale in commit messages. CoMRAT enables a) researchers to produce metrics and analyses on rationale information in any Github module, and b) developers to check the amount of rationale in their commit messages. A preliminary evaluation suggests the tool's usefulness and usability in both these research and development contexts.

==> text/analysis_evolution.tex <==



%%%%%%%%%%%%%%%
\begin{figure*}[p]
 \begin{subfigure}{0.9\textwidth}
     \includegraphics[width=\textwidth]{figures/evolution_decision_rationale_slob.pdf}
     \caption{Slob}
     \label{fig:evolution_decision_rationale_slob}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.9\textwidth}
     \includegraphics[width=\textwidth]{figures/evolution_decision_rationale_button.pdf}
     \caption{Button}
     \label{fig:evolution__decision_rationale_button}
 \end{subfigure}
 
 \medskip
 \begin{subfigure}{0.9\textwidth}
     \includegraphics[width=\textwidth]{figures/evolution_decision_rationale_fs.pdf}
     \caption{Fs}
     \label{fig:evolution__decision_rationale_fs}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.9\textwidth}
     \includegraphics[width=\textwidth]{figures/evolution_decision_rationale_migrate.pdf}
     \caption{Migrate}
     \label{fig:evolution_decision_rationale__migrate}
 \end{subfigure}

 \caption{Yearly evolution of the average rationale density and the average decision density }
 \label{fig:decision_rationale_evolution}

\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%



==> text/analysis_factors.tex <==


% 1. A normality test on the distribution of the  rationale density of the commits :  \\
% mm: (p\_value = 0.02 $<$ 0.05). \\
% slob:  (p\_value =  0.06 $>$ 0.05). \todo{} \\
% button:  (p\_value = 0.31  $>$ 0.05). \todo{} \\
% fs: (p\_value =  0.36 $>$ 0.05).  \todo{} \\
% migrate:   (p\_value = 0.001  $<$ 0.05).  \\

% %%%%
% 2. A normality test on the distribution for
% the commit messages sizes :  \\ 
% mm: (p\_value = $ 1.73e-55 <$ 0.05).  \\
% slob:   (p\_value =  1.47e-33  $<$ 0.05).   \\
% button:(p\_value =  2.26e-3 $<$ 0.05).  \\
% fs:(p\_value =  4.34e-06 $<$ 0.05).  \\ 
% migrate:(p\_value = 4.63e-140  $<$ 0.05). \\

% %%%%
% Since both distributions are not normal, we use Spearman’s rank correlation coefficient to discover whether or not there is a correlation between the commit message size and its rationale density:\\ 

% mm: (p\_value = $ 2.45e-10 $ $<$ 0.05,  R = $ - 0.32 $). \\
% slob: (p\_value = 0.25  $>$ 0.05, R = 0.095 ). \todo{?}
% \\
% button: (p\_value = 0.82  $>$ 0.05,  R = 0.021 ). \todo{?}  \\

% fs: (p\_value = 0.71  $>$ 0.05,  R = -0.10).  \todo{?} \\ 

% migrate: (p\_value =  0.4 $>$ 0.05,  R = -0.03 ). \todo{?} \\


% Results indicate that there is no \todo{??}correlation between them.




%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}[p]
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_over_size_slob.pdf}
     \caption{Slob}
     \label{fig:rationale_density_over_size_slob}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_over_size_button.pdf}
     \caption{Button}
     \label{fig:rationale_density_over_size_button}
 \end{subfigure}
 
 \medskip
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_over_size_fs.pdf}
     \caption{Fs}
     \label{fig:rationale_density_over_size_fs}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_over_size_migrate.pdf}
     \caption{Migrate}
     \label{fig:rationale_density_over_size_migrate}
 \end{subfigure}

 \caption{Commit message size versus rationale density}
 \label{Label}

\end{figure*}

%%%%%%%%%%%


% The normality test result indicates that the  number of commits per author is not a normal distribution:\\

% mm: ($p\_value=4.45e^{-33} < 0.05$). \\
% slob: ($p\_value= ?? < 0.05$). \\
% button: ($p\_value= ?? < 0.05$). \\
% fs: ($p\_value= ??  < 0.05$). \\
% migrate: ($p\_value= ??  < 0.05$). \\

% Spearman's rank correlation coefficient between  the number of commits per author and the average \textit{rationale density} per author indicates that the test is not significant : 

% mm: ($ p\_value=0.635 > 0.05, R =- ?? $).\\
% slob: ($ p\_value= ?? > 0.05, R = ?? $).. \\
% button:($ p\_value= ?? > 0.05, R = ?? $). \\
% fs: ($ p\_value= ?? > 0.05, R = ?? $).. \\
% migrate: ($ p\_value= ?? > 0.05, R = ?? $). \\


%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[p]
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_per_author_slob.pdf}
     \caption{Slob}
     \label{fig:rationale_density_per_author_slob}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_per_author_button.pdf}
     \caption{Button}
     \label{fig:rationale_density_per_author_button}
 \end{subfigure}
 
 \medskip
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_per_author_fs.pdf}
     \caption{Fs}
     \label{fig:rationale_density_per_author_fs}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/rationale_density_per_author_migrate.pdf}
     \caption{Migrate}
     \label{fig:rationale_density_per_author_migrate}
 \end{subfigure}

 \caption{Commits per author vs average rationale density}
 \label{Label}

\end{figure*}





==> text/analysis_structure.tex <==


%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[p]
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/commit_strcuture_normalizedslob.pdf}
     \caption{Slob}
     \label{fig:commit_strcuture_normalized_slob}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/commit_strcuture_normalizedbutton.pdf}
     \caption{Button}
     \label{fig:commit_strcuture_normalized_button}
 \end{subfigure}
 
 \medskip
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/commit_strcuture_normalized_fs.pdf}
     \caption{Fs}
     \label{fig:commit_strcuture_normalized_fs}
 \end{subfigure}
 \hfill
 \begin{subfigure}{0.49\textwidth}
     \includegraphics[width=\textwidth]{figures/commit_strcuture_normalized_migrate.pdf}
     \caption{Migrate}
     \label{fig:commit_strcuture_normalized_migrate}
 \end{subfigure}

 \caption{Category distribution over the normalized positions
of commit message sentences (considering overlap)}
 \label{Label}

\end{figure*}

%%%%%%%%%%%%%%%%%%



==> text/threats.tex <==
\section{Threats To Validity}
\label{sec:threats}
%In this section, we present the potential
%threats that could hamper the validity of our study and the  steps we took to mitigate them.

\todo{rephrase, now copy/pate}

\textbf{Construct validity.}
The measures we use to identify the presence of the different categories in the commits (i.e, the \textit{densities}), are quantitative measures. We do not measure this presence qualitatively. In fact,  we are not aware of any qualitative measures of rationale or decisions. Furthermore, we consider the number of commits written as an indicator of author experience. 
%Although t
This is not necessarily true.
The number of commits is also computed as an overall classification for the author and not at the time of the commit. This introduces a threat as  authors might have gained experience during the studied period. However,
our findings mitigate this threat as we can see a clear difference between the authors with several commits and the authors with few commits (Figure~\ref{fig:rationale_density_per_author}). Thus, the data leads us to believe that the number of commits authored is a reasonable measure of experience. 

\textbf{Internal validity.}
We only studied commits that were approved by the Linux maintainers, which could introduce survivor bias. 
This is acceptable as we are interested in the rationale of the software as it is, not as it could have been. Comparing our findings with the characteristics of rationale in rejected commits is however an interesting research question for the future. 
Additionally, some metrics are calculated based on a low number of commits (e.g. some monthly and yearly averages when studying rationale evolution). This represents a threat as it may mean that the results are more metrics of a few particular commits rather than true evolutionary trends.

\textbf{External validity.} 
We only studied the commit history that is available on Git. Our observations might not be applicable to contributions in the earlier years of Linux.

Additionally, there is no reason to assume that our findings can be extrapolated to other OSS  projects.
In fact, we note that while there are real differences between the way contributions are managed in Linux compared to other large OSS projects, there are also lessons to be learned across projects~\cite{bettenburg2015management}. We view this paper as a step towards creating a better understanding of rationale in OSS generally, which can lead to improvements in automatic rationale extraction across projects.





